Thinking Outside the Lab: VR Size & Depth Perception in the Wild

Size and distance perception in Virtual Reality (VR) have been widely studied, albeit in a controlled laboratory setting with a small number of participants. We describe a fully remote perceptual study with a gamified protocol to encourage participant engagement, which allowed us to quickly collect high-quality data from a large, diverse participant pool (N=60). Our study aims to understand medium-field size and egocentric distance perception in real-world usage of consumer VR devices. We utilized two perceptual matching tasks -- distance bisection and size matching -- at the same target distances of 1--9 metres. While the bisection protocol indicated a near-universal trend of nonlinear distance compression, the size matching estimates were more equivocal. Varying eye-height from the floor plane showed no significant effect on the judgements. We also discuss the pros and cons of a fully remote perceptual study in VR, the impact of hardware variation, and measures needed to ensure high-quality data.

==> 99_citation_backup.tex <==

\gs{New size comp papers}\\

Kim et al.~\cite{kim2017dwarf} (VR, eye height, size)
    \begin{itemize}
        \item found that size judgments were moderately correlated (r = 0.4) between the two response methods, and that neither altered eye height ($\pm 50cm$) nor reduced ($10mm$) interpupillary distance (IPD) had a significant effect on size judgments, but that a wider (150mm) IPD caused a significant ($\mu = 38\%, p < 0.01$) decrease in perceived cube size.
    \end{itemize}
    
Combe et al.~\cite{combe20081}\\
    Experiment: compare 1:1 scale perception in these two devices in reference to physical 1:1 scale of the vehicle cockpit (i.e. the object)
    \begin{itemize}
        \item We show that differences exist between size perception using the HMD, and using the cylindrical screen. Underestimations seem to be more frequent when using cylindrical screen.Moreover, the level of knowledge of the vehicle and the virtual reality system also seems to influence subject’s size perception.
    \end{itemize}

\gs{end}\\

\gs{New bisection papers}\\

Hornsey et al.~\cite{hornset2017distance} (VR)
    \begin{itemize}
        \item accurate and there was no evidence of distance compression for distances of between 1 and 10m
    \end{itemize}

Gamberini et al.~\cite{gamberini2013behavioural}. (real world, use laser pointer)
    \begin{itemize} 
        \item The results showed that distance moderated the effect of action. At an unreachable distance(120cm), the mean bisection point was closer to the centre when participants used the laser cutter compared to when they used the laser pointer. There were no differences at a reachable distance (60 cm).
    \end{itemize}

\gs{end}\\

Oberfeld et al.~\cite{oberfeld2010surface}. (VR, wall lightness and height perception)
    \begin{itemize}
        \item the perceived height additionally increased with wall lightness, and the effects of wall lightness and ceiling lightness were roughly additive, incompatible with a simple effect of the lightness contrast between the ceiling and the walls.
        \item the floor lightness has no significant effect on perceived height, and that the total brightness of the room is not the critical factor influencing the perceived height.
    \end{itemize}
    
    
Glennerster et al.~\cite{glennerster2006humans}. (VR, \textbf{size judgement})
    \begin{itemize}
        \item failed to notice when a scene expanded or contracted, despite having consistent information about scale from both distance walked and binocular vision.
        \item the efficacy of motion and disparity cues is greater at near viewing distances
        \item observers more willing to adjust their estimate of interocular separation or distance walked than to accept that the scene has changed in size
    \end{itemize}
    
    
Peillard et al.~\cite{peillard2019virtual}. (VR, depth perception, orientation)
    \begin{itemize}
        \item the orientation of virtual stimuli with respect to the user introduces a distance perception bias: objects placed on the sides are systematically perceived farther away than objects in front
        \item this bias increases along with the angle, and appears to be independent of both the position of the object in the field of view as well as the quality of the virtual scene
    \end{itemize}
    
Naceri et al.~\cite{naceri2015depth}. (real world + VR, control visual size)
\begin{itemize}
    \item In the real environment, all participants perceived the depth of the target object precisely. Whereas, in virtual reality (VR) the responses were significantly less precise, although, still above chance level in 16 of the 20 observers.
\end{itemize}

Li et al.~\cite{li2016the}. (VR, frame, FOV, depth)
    \begin{itemize}
        \item provides evidence that the device FOV and peripheral light could influence distance judgments in HMDs
        \item the degree of influence might not change proportionally with respect to the peripheral light brightness.
    \end{itemize}
    
Maruhn et al.~\cite{maruhn2019measuring}. (VR, depth, methodologies, locomotion, translation gains)
\begin{itemize}
    \item significant differences between methods were observed, with the smallest error occurring for visually guided walking and verbal estimates. 
    \item non-visual cues during walking affected distance estimates. This relationship was mainly evident for methods building on actual or imagined walking movements and verbal estimates.
\end{itemize}

Renner et al.~\cite{renner2013the}. (VR, egocentric depth)
    \begin{itemize}
        \item it is important to provide binocular disparity, use high quality of graphics, carefully adjust the virtual camera settings, display a rich virtual environment containing a regularly structured ground texture, and enhance the user’s sense of presence
    \end{itemize}

Hornsey et al.~\cite{hornsey2020size}. (VR, \textbf{size}, shape)
    \begin{itemize}
        \item show under-constancy, such that the apparent size and depth both tend to reduce with increasing distance.
    \end{itemize}

Corujeira et al.~\cite{corujeira2013stereocopic}. (VR, egocentric depth, eye height, device)
    \begin{itemize}
        \item  substantial under-estimation of distance across all conditions
        \item low eye-height led to a significant reduction in the level of underestimation in the HMD and 3D Stereo Display
        \item No significant effect between Display conditions (HMD and 3D monitor and Restricted Real World)
    \end{itemize}
    
Cidota et al.~\cite{cidota2016using} (AR + VR, depth)
\begin{itemize}
    \item visual effects both in AR and VR have a negative impact on perceived depth
    \item the measured performance in VR though is best using visual effects while in AR without using visual effects
\end{itemize}

Anil et al.~\cite{anil2019do} (AR + VR, 3D pointing on close-by target)
    \begin{itemize}
        \item subjects' movements towards/away from their head were slower and less accurate than their lateral movements
        \item moved faster in AR, no significant difference for pointing performance
    \end{itemize}
    
Kelly et al.~\cite{kelly2004perception} (real world vs. VR)
Experiment:
     Participants indicated which parts of the scene were visible to an assistant or avatar (simulated person used in virtual environments) and which parts were occluded by a nearby building
\begin{itemize}
    \item Errors increased with increasing distance between the participant and the assistant out to 15 m, and error patterns were similar between real and virtual environments
    \item similarity is especially interesting given recent reports that environmental geometry is perceived differently in virtual environments than in real environments.
\end{itemize}
    
%Loomis et al.~\cite{loomis2003visual} (real world, VR, egocentric distance)
    %\\
%    \textbf{Did not find anything new/interesting... This book seems more like a summary to me}
    
\subsubsection{AR}
Singh et al.~\cite{singh2010depth} (Near-field AR(34-50cm))
    \begin{itemize}
        \item found maximum average depth judgment errors of 5.5 cm, and found that the blind reaching judgments were less accurate than the perceptual matching judgments. 
        \item found that the presence of a highly-salient occluding surface has a complicated effect on depth judgments, but does not lead to systematically larger or smaller errors. 
    \end{itemize}


Diaz et al.~\cite{diaz2017designing} (AR, egocentric depth)
    \begin{itemize}
        \item On average, viewers underestimated virtual object depth
        \item cast shadows appear highly beneficial for depth estimation
        \item Design combinations interacted in complex ways, potentially improving the perceived depth of virtual objects in the real world over individual design choices
    \end{itemize}



Serefoglou et al.~\cite{serefoglou2008hand} (video see-through HMD, height, hand-eye coordination)
    \begin{itemize}
        \item A significant decrease in accuracy was found compared to  direct view
        \item cameras should be placed above or below eye level, but by no more than 35 mm, in order to preserve hand-eye coordination
    \end{itemize}

Franco et al.~\cite{franco2019augmented} (AR, methodology)
    \begin{itemize}
        \item users' felt more comfortable using a familiar handheld controller
        \item the solution with the smart glass's tap function and head movement got results close to the results of smart glass's controller
    \end{itemize}

Edward et al.~\cite{edwards1993video} (video see-through optical system design and system consideration)
    \begin{itemize}
        \item  two miniature video cameras must ideally simulate the eyes of the person wearing the helmet - should be positioned with respect to the HMD as if  they occupy the eyes physical locations
        \item  reduction in vertical FOV while maintaining perfect position of the cameras will present an easier to adapt display for the wearer.
    \end{itemize}

Iwamoto et al.~\cite{iwamoto2013high} (binocular video see-through display, high resolution, interactive work support)
    \begin{itemize}
        \item this paper constructed a high-resolution video see-through display for interactive work support.
        \item the depth perception of operator was evaluated, high accuracy.
        \item peg insertion experiment was evaluated, work efficiency is improved compared with the results of the monocular display system
    \end{itemize}

Swan et al.~\cite{swan2007egocentric} (optical see-through AR, egocentric distance)
    \begin{itemize}
        \item the egocentric depth of AR objects is underestimated at these distances, but to a lesser degree than has previously been found for most virtual reality environments. 
        \item the results are consistent with previous studies that have implicated a restricted field-of-view, combined with an inability for observers to scan the ground plane in a near-to-far direction, as explanations for the observed depth underestimation.
    \end{itemize}
